Simulated Blockchains for Machine Learning Traceability and Transaction Values in the Monero Network

Monero is a popular crypto-currency which focuses on privacy. The blockchain uses cryptographic techniques to obscure transaction values as well as a `ring confidential transaction' which seeks to hide a real transaction among a variable number of spoofed transactions. We have developed training sets of simulated blockchains of 10 and 50 agents, for which we have control over the ground truth and keys, in order to test these claims. We featurize Monero transactions by characterizing the local structure of the public-facing blockchains and use labels obtained from the simulations to perform machine learning. Machine Learning of our features on the simulated blockchain shows that the technique can be used to aide in identifying individuals and groups, although it did not successfully reveal the hidden transaction values. We apply the technique on the real Monero blockchain to identify ShapeShift transactions, a cryptocurrency exchange that has leaked information through their API providing labels for themselves and their users.

==> snippets_ana_005/snippet_correlations_lihan.tex <==

Lihan 12:27 PM
For an empirical dist X, mix-in Z, and real Y we have  X = (10/11)Z + (1/11)Y. For a histogram binning scheme c, we want to recover the histogram Y'^c of the denoised data Y'. I think (or a proof is needed) X^c = (120/121)Z'^c + Y'^c, where we have knowledge of X^c, and Z'^c by our knowledge Z. In inference, we predict the input pair (x_1,x_2) of maximum likelihood from Y'^c (edited) 
12:32 PM
and this would be valid for blocks of the recent mix-in procedure. (edited) 

Lihan 1:05 PM
residual (relative entropy among distributions) between empirical and proposed mixin within the tracebility paper hasn't been used. We Compute the KL-divergence D( mixin || their empirical ) . Now we know the 'surprise' that their empirical dist introduces (entropy un-explained by the mixin). We propose a Y' such that D( mixin || their empirical ) = D( mixin || Y' ). This may be the compelling validation that Y'^c needs: our recovered signal is the same earth-mover distance as the unexplained entropy in their empirical analysis. (edited) 

